Contextual bandits with surrogate losses: Margin bounds and efficient algorithms

We use surrogate losses to obtain several new regret bounds and new algorithms for contextual bandit learning. Using the ramp loss, we derive new margin-based regret bounds in terms of standard sequential complexity measures of a benchmark class of real-valued regression functions. Using the hinge loss, we derive an efficient algorithm with a $\sqrt{dT}$-type mistake bound against benchmark policies induced by $d$-dimensional regressors. Under realizability assumptions, our results also yield classical regret bounds.

==> main.tex <==
\section{Introduction}
We study sequential prediction problems with partial feedback,
mathematically modeled as \emph{contextual bandits}. In this
formalism, a learner repeatedly (a) observes a \emph{context}, (b)
selects an \emph{action}, and (c) receives a \emph{loss} for the
chosen action. The objective is to learn a policy for selecting
actions with low loss, formally measured via a notion of regret with
respect to a large class of benchmark policies.  Contextual bandit
algorithms have been successfully deployed in online recommendation
systems, mobile health platforms, and elsewhere.

In this paper, we use surrogate loss functions to derive new
algorithms and regret bounds for contextual bandits. Surrogate loss
functions are ubiquitous in supervised and online learning.
Computationally, they can make NP-hard optimization problems
computationally tractable, e.g., the logistic loss makes binary
classification amenable to convex programming
techniques. Statistically, they also enable sharper generalization
analysis, e.g., margin-based analyses for boosting, SVM, and neural
networks. Curiously, surrogate losses have seen limited use in partial
information settings.  This paper demonstrates that these desirable
computational and statistical properties extend to contextual bandits.

% Curiously, apart from research on bandit
% multiclass prediction, which we discuss in the sequel, surrogate
% losses have seen limited use in partial information settings.  

% This
% paper demonstrates that surrogate loss functions have desirable
% statistical and computational properties for contextual bandits,
% analogously to statistical learning.

In the first part of the paper, we focus on statistical issues and
derive a new margin-based regret bound for adversarial contextual
bandits. We consider benchmark policies induced by a class $\Fcal$ of
real-valued regressors, and our regret bound involves standard
sequential complexity measures of $\Fcal$. These results considerably
generalize prior bounds for contextual bandits, almost all of which
focus on the finite-class case. Technically, our approach here employs
the ramp loss in the adaptive minimax framework of Foster et
al.~\cite{FosRakSri15} along with a careful chaining argument.

In the second part of the paper, we focus on computational issues and
derive two new algorithms, using the hinge loss as a convex
surrogate. The first algorithm provably runs in polynomial time and
achieves $\sqrt{T}$-type mistake bound in a variety of settings, which
can be converted to a standard regret bound under realizability
assumptions. This algorithm is based on the Exponential-Weights
update, using Langevin Monte Carlo for efficient sampling, and with a
careful action selection scheme to ensure low regret.  The second
algorithm is much simpler; we show that Follow-The-Leader with uniform
smoothing achieves the optimal regret when the class $\Fcal$ is
sufficiently large.


\section{Preliminaries}
Let $\Xcal$ denote a context space and let $\Acal = \{1,\ldots,K\}$
denote a discrete action space. In the adversarial contextual bandits
problem, for each of $T$ rounds, an adversary chooses a pair
$(x_t,\ell_t)$ where $x_t \in \Xcal$ is the context, and $\ell_t \in
[0,1]^K$ is a loss vector, then the learner observes the context
$x_t$, chooses an action $a_t$, and incurs loss $\ell_t(a_t) \in
[0,1]$, which is also observed. The goal of the learner is minimize
the cumulative loss over the course of the $T$ rounds, and, in
particular, we would like to design learning algorithms that achieve
low \emph{regret} against a class $\Pi \subset \Xcal \to \Acal$ of
benchmark policies:
\begin{align*}
  \Reg(T,\Pi) = \sum_{t=1}^T\EE[\ell_t(a_t)] - \inf_{\pi \in \Pi} \sum_{t=1}^T \EE[\ell_t(\pi(x_t))].
\end{align*}

In this paper, we always identify the policy class $\Pi$ with a class
of vector-valued regression functions $\Fcal \subset (\Xcal \to
\RRz^K)$, where we define $\RRz^K \triangleq \{s \in \RR^K: \sum_a s_a = 0\}$. For
such functions, we use the notation $f(x) \in \RR^K$ to denote the
vector-valued output, and $f(x,a)$ to denote the $a^{\textrm{th}}$
component.  Note that we are assuming $\sum_a f(x,a) = 0$ which can be easily arranged.
%% Without loss of generality, we assume that for all $f \in
%% \Fcal, x \in \Xcal, \sum_{a}f(x,a) = 0$, which can be easily arranged.

All of our algorithms use \emph{importance weighting} to form unbiased
loss estimates. If at round $t$, the algorithm chooses its action
$a_t$ by sampling from a distribution $p_t \in \Delta(\Acal)$, the
importance weighted loss estimate is defined as
$\hat{\ell}_t(a) \triangleq \ell_t(a_t)\one\{a_t=a\}/p_t(a)$. Often we
will also apply a smoothing operation defining a smoothed distribution
as $p_t^\mu \triangleq (1-K\mu)p_t + \mu$ for some parameter
$\mu \in [0,1/K]$.


We introduce two surrogate loss functions, the \emph{ramp loss} and
the \emph{hinge loss}. Let $\ramp(s) \triangleq
\min(\max(1+s/\gamma,0),1)$ denote the scalar ramp loss and let
$\hinge(s) \triangleq \max(1+s/\gamma,0)$ denote the scalar hinge
loss. We start with a simple lemma, demonstrating how $\ramp,\hinge$
can act as surrogate losses.

\begin{lemma}[Surrogate Loss Calibration]
\label{lem:calibration}
For $s \in \RRz^K$ define $\piramp(s) \in \Delta([K])$ by
$\piramp(s)_a \propto \ramp(s_a)$ and define $\pihinge(s)$
analogously. For any vector $\ell \in \RR^K_+$, we have
\begin{align*}
  \langle \piramp(s), \ell\rangle &\leq \langle \ell,\ramp(s)\rangle \leq \sum_{a \in \Acal}\ell(a)\one\{s_a \ge -\gamma\}, \qquad
  \langle \pihinge(s), \ell\rangle \leq K^{-1} \langle \ell,\hinge(s)\rangle.
\end{align*}
\end{lemma}


\paragraph{Related Work.}
Contextual bandit learning has been the subject of intense
investigation over the past decade. These works come in several
flavors, but the most natural categorization of the theoretical works
is between parametric and agnostic approaches. The parametric methods
(c.f.~\cite{abbasi2011improved,chu2011contextual}) assume that the
losses are related to the contexts and actions through a known
functional form (e.g., linear) and measure regret relative to a
globally optimal policy. In contrast, the agnostic approaches
(c.f.~\cite{agarwal2014taming}) avoid such parametric assumptions and
instead compete with a restricted policy class for statistical
tractability. In this latter setting, most results for efficient
algorithms require stochasticity assumptions, although some recent
work has been focusing on the adversarial case.  This work contributes
to all of these directions; our margin bounds apply to the agnostic
adversarial setting, and yield true regret bounds under parametric or
realizability assumptions.

A special case of the contextual bandit problem is \emph{bandit
  multiclass prediction}, in which the loss vector is zero for one
action, and one for all others. Several recent papers derive surrogate
regret bounds for this setting, when the benchmark policy class
$\Fcal$ consists of linear functions of the context. Our work
contributes to this line in two ways: we design new loss functions
that yield efficient algorithms with surrogate regret bounds for the
general contextual bandit case, and we extend beyond linear/parametric
benchmark classes.

Surrogate losses and margin bounds are prevalent in statistical and
online learning. The most obvious advantage is computational, since a
surrogate loss can make a discrete optimization problem continuous and
even convex, and idea that has been exploited in the bandit multiclass
literature. Yet, surrogate losses also offer statistical advantages as
well; margin bounds provide a more accurate characterization of the
generalization performance of boosting and neural networks. Here we
show that both of these properties arise in contextual bandits as
well.

At a technical level, our work incorporates a number of statistical
and algorithmic ideas from the literature. To derive achievable regret
bounds, we use the adaptive minimax framework of Foster et
al.~\cite{FosRakSri15}, along with a novel chaining
argument~\cite{Dudley84} to control the fluctuations of a martingale
process~\cite{liang2015learning}. The core of the algorithm is based
on log-concave sampling~\cite{bubeck2015sampling}, but also involves
other components, including randomized
smoothing~\cite{duchi2012randomized}, the geometric resampling trick
of Neu. We also use several ideas from the classification calibration
literature, and in particular our surrogate loss functions are studied
by Pires et al.~\cite{pires2013cost}.


\section{Achievable regret bounds}
\label{sec:minimax}
In this section we develop a new family of regret bounds for
adversarial contextual bandits. The departure point for our approach
is a well known reduction from bandits to full information problems:
If a full information algorithm achieves a regret bound in terms of
the \emph{local norms} $\sum_t\langle p_t,\ell_t^2\rangle$, then
running the full information algorithm on importance weighted losses
yields an expected regret bound for the bandit setting. For example,
EXP4 exploits this observation for the case when $\Pi$ is finite,
using Hedge as the full information algorithm, and obtaining an
expected regret bound of
\begin{align*}
\Reg(T,\Pi) \leq \frac{\eta}{2} \sum_{t=1}^T \EE[\langle p_t, \hat{\ell}_t^2\rangle] + \frac{\log (|\Pi|)}{\eta}.
\end{align*}
Evaluating the expectation and optimizing the learning rate $\eta$
yields an optimal $\order(\sqrt{KT\log(|\Pi|)})$ regret bound for this
setting.  Moving beyond the finite class case, when are such
local-norm bounds achievable?

\section{Efficient Algorithms}
\label{sec:algorithms}

This section contains two new algorithmic guarantees for contextual
bandits, both using the hinge loss $\hinge$ defined in
Section~\ref{sec:prelims}. The first algorithm focuses on a parametric
class of real-valued regressors; it is based on a continuous version
of Exponential Weights using a log-concave sampler and we call this
algorithm \lmc, with the description and guarantees provided in
Subsection~\ref{ssec:hinge_lmc}. The second algorithm is simple
follow-the-leader with uniform smoothing, which we call \ftl,
described in Subsection~\ref{ssec:ftl}.


\subsection{Hinge-LMC}
\label{ssec:hinge_lmc}
For this section, we identify $\Fcal$ with a compact convex set
$\Theta\subset \RR^d$, using the notation $f(x;\theta) \in \RRz^K$, to
describe the parametrized function. We further assume that
$f(x;\theta)$ is convex in $\theta$ for each $x$,
$\sup_{x,\theta}\|f(x;\theta)\|_{\infty}\leq B$, $f(x,a;\cdot)$ is
$L$-Lipschitz as a function of $\theta$ with respect to $\ell_{2}$
norm for each $x,a$, and that $\Theta$ contains the centered Euclidean
ball of radius $1$, and is contained within a Euclidean ball of radius
$R$. The pseudocode for the algorithm, \lmc, is displayed in
Algorithm~\ref{alg:hinge_lmc}, with a sampling subroutine in
Algorithm~\ref{alg:lmc}.

\begin{figure*}
\begin{minipage}{0.5\linewidth}
\begin{algorithm}[H]
\begin{algorithmic}
  \State Define $w_0(\theta) = 1$ for all $\theta \in \Theta$.
  \For{$t = 1,\ldots,T$}
  \State Receive $x_t$
  \State $\theta_{t} \gets $ LMC($\eta w_{t-1}$), set $p_t \propto \hinge(f(x_t;\theta_t))$
  \State Set $p^\mu_t = (1-K\mu)p_t + \mu$.
  \State Play $a_t \sim \tilde{p}_t$, observe $\ell_t(a_t)$.
  \For{$m = 1,\ldots,M$}
  \State $\tilde{\theta}_t \gets $ LMC($\eta w_{t-1}$).
  \State Sample $\tilde{a}_t \sim p^\mu_t(\tilde{\theta}_t)$, if $\tilde{a}_t = a_t$, break
  \EndFor
  \State Set $\tilde{\ell}_t(a) = m\ell_t(a_t)\one\{a_t = a\}$
  \State Update $w_{t}(\theta) \gets \langle \tilde{\ell}_t, \hinge(f(x_t;\theta))\rangle$
  \EndFor
\end{algorithmic}
\caption{\lmc}
\label{alg:hinge_lmc}
\end{algorithm}
\end{minipage}
\begin{minipage}{0.5\linewidth}
\begin{algorithm}[H]
\begin{algorithmic}
    \State Input: Function $F$, parameters
    $m,u,\lambda,N,\alpha$.
    \State Set $\tilde{\theta}_k \gets 0 \in \RR^d$
    \For{$k = 1,\ldots,N$}
    \State Draw $z_1,\ldots,z_m \iidsim \Ncal(0, u^2 I_{d})$ and define
    \begin{align*}
      \tilde{F}_k(\theta) = \tfrac{1}{m}\textstyle\sum\nolimits_{i=1}^m F(\theta+z_i) + \lambda \|\theta\|_2^2
    \end{align*}
    \State Draw $\xi_k \sim \Ncal(0,I_d)$ and update
    \begin{align*}
      \tilde{\theta}_{k} \gets \Pcal_{\Theta}\left(\tilde{\theta}_{k-1} - \alpha \nabla \tilde{F}_k(\tilde{\theta}_{k-1}) + \sqrt{2\alpha}\xi_k\right).
    \end{align*}
    \vspace{-0.07cm}
    \EndFor
    \State Return $\tilde{\theta}_N$. 
\end{algorithmic}
\caption{Langevin Monte Carlo (LMC)}
\label{alg:lmc}
\end{algorithm}
\end{minipage}
\end{figure*}

The main idea is to simply run exponential weights on the surrogate
hinge loss. At round $t$, we define the exponential weights
distribution via its density (w.r.t. the Lebesgue measure over
$\Theta$)
\begin{align*}
P_t(\theta) \propto \exp(-\eta w_{t-1}(\theta)) \qquad w_{t-1}(\theta) = \sum_{s=1}^{t-1}\langle \tilde{\ell}_s, \hinge(f(x_s;\theta))\rangle,
\end{align*}
where $\eta$ is a learning rate, and $\tilde{\ell}_s$ is an estimate
of the loss vector. At a high level, at each iteration the algorithm
generates a sample $\theta_t \sim P_t$, and then samples action $a_t$
from the induced policy distribution $\pihinge(f(x_t;\theta_t))
\propto \hinge(f(x;\theta)) \in \Delta(\Acal)$. It then plays $a_t$,
observes the loss $\ell_t(a_t)$, and constructs a loss vector estimate
$\tilde{\ell}_t = m_t\ell_t(a)\one\{a = a_t\}$ where $m_t$ is computed
by repeatedly sampling from $P_t$. This vector $\tilde{\ell}_t$ is
passed to the Hedge subroutine to define the distribution at the next
round. To generate samples $\theta_t \sim P_t$ we use Projected
Langevin Monte Carlo.

Each of these components has many subtleties that are important for
the both statistical and computational guarantee, which we describe in
detail in the appendix. Here, we state the main guarantee and its
consequences.
\begin{theorem}
  \label{thm:hinge_lmc}
  Under the assumptions above, Algorithm~\ref{alg:hinge_lmc}, with
  parameters $\eta,\gamma,M,\mu$, guarantees
  \begin{align*}
    \EE \sum_{t=1}^T \ell_t(a_t) \leq \inf_{\theta \in \Theta} \frac{1}{K}\EE \sum_{t=1}^T\langle \ell_t, \hinge(f(x_t;\theta))\rangle + O\left(\frac{B}{\gamma}\sqrt{dT}\right).
  \end{align*}
  Moreover, the algorithm runs in $\poly(T,d,B,\gamma,R,L)$ time.
\end{theorem}

Since Bandit Multiclass Classification is a special case of Contextual
Bandits, Theorem~\ref{thm:hinge_lmc} immediately implies a
$\sqrt{dT}$-mistake bound for this setting.
\begin{corollary}[Bandit Multiclass]
  \label{cor:bandit_multiclass}
  In the bandit multiclass setting, Algorithm~\ref{alg:hinge_lmc}
  enjoys a mistake bound of $\otil(\frac{B}{\gamma}\sqrt{dT})$ and
  runs in polynomial time.
\end{corollary}

Additionally, under a calibration/realizability condition for the
hinge loss, we obtain a standard regret bound via an efficient
algorithm. For simplicitly in defining the condition, assume that for
every $(x,\ell)$ pair, $\ell$ is a random variable with conditional
mean $\bar{\ell}$ (chosen by the adversary) and $\bar{\ell}$ has a unique action
with minimal loss.
\begin{corollary}[Calibrated CB]
  \label{cor:realizable}
  In addition to the conditions above, assume that there exists
  $\theta^\star \in \Theta$ such that for every $(x,\ell)$ pair chosen
  by the adversary, we have $f(x,a;\theta^\star) =
  K\gamma\one\{\bar{\ell}(a) \leq \min_{a'}\bar{\ell}(a')\} -
  \gamma$. Then \lmc\xspace with the same parameters as in
  Theorem~\ref{thm:hinge_lmc} guarantees $\Reg(T,\Theta) \leq
  \otil(B/\gamma\sqrt{dT})$ regret and runs in polynomial time.
\end{corollary}

%% Before turning to a more detailed description of the algorithmic
%% components, there are many points work making:
A few comments are in order:
\begin{packed_enum}
\item While the algorithm is guaranteed to run in polynomial time, the
  dependence on $T,d$ that we obtain is quite poor. In part this
  inefficiency stems from the mixing-time analysis for Projected
  LMC~\cite{bubeck2015sampling}. More recent results in slightly
  different settings~\cite{raginsky2017non} suggest that this analysis
  can be improved, and even extended to non-convex settings.
%% \item Indeed, we view \lmc and Theorem~\ref{thm:hinge_lmc} as
%%   justification for the Bagging algorithm, which uses several copies
%%   of gradient descent trained with small variations of the history to
%%   form a distribution over parameters. This closely resembles \lmc, In
%%   a recent empirical evalution, Bagging was shown to be
\item Corollary~\ref{cor:bandit_multiclass} provides a new solution to
  the open problem of Abernethy and Rakhlin~\cite{abernethyR09a}. In
  fact, this result is the first that uses a true hinge loss, although
  it is different from the standard multiclass hinge loss, used by
  \citet{kakade2008efficient} in a $T^{2/3}$-regret algorithm. All
  prior $\sqrt{T}$-regret
  algorithms~\cite{hazan2011newtron,beygelzimerOZ17,foster2018logistic}
  use different losses, e.g., the multiclass logistic loss, and in
  particular rely on differentiability and smoothness.
\item 
%% It is somewhat curious that the regret bounds have no explicit
%%   dependence on $K$, but note that the appropriate scaling is $B \ge
%%   K\gamma$. More concretely, 
  Note that for Corollary~\ref{cor:realizable}, a requirement for the
  realizability condition is that $B \ge K\gamma$, and hence the
  dependence on $K$ is implicit.
\item For Corollary~\ref{cor:realizable}, the best points of
  comparison are EXP4, oracle based methods, and methods based on
  square-loss realizability. EXP4 and oracle-based methods are not
  computationally efficient in this setting since the effective policy
  class is exponentially large and the oracle solves an NP-hard
  problem. In comparison with the latter family, our approach
  considers general convex parametrizations and yields better regret
  guarantees than those in~\citet{foster2018practical}.
%% To provide a point of comparison, we could
%%   discretize the space $\Theta$ and run EXP4 on the discretization to
%%   obtain a regret bound of $\otil(\sqrt{KdT})$, even without the
%%   realizability condition. However, the running time of this latter
%%   algorithm is exponential in $d$, since one will have to maintain a
%%   distribution over exponentially many parameters.
%% \item The other points of comparison here are oracle-based approaches, and
%%   approaches based on square-loss realizability. While the former
%%   family does not require any realizability assumptions, the
%%   algorithms technically require solving problems that NP-hard in the
%%   worst case, and further, it is not known how to achieve
%%   $\sqrt{T}$-regret when the contexts are adversarially generated,
%%   even with realizability. The latter class of algorithms use a
%%   different notion of realizability, which is intuitively similar, but
%%   actually more difficult statistically, as discussed above. Moreover,
%%   our work considers general convex parametrizations, and yields
%%   better regret guarantees than those in Foster et
%%   al.~\cite{foster2018practical}.
\end{packed_enum}

\begin{comment}
We now briefly describe the main computational and statistical
insights. 
%% Computationally, the main insight is that by using the hinge
%% loss, $P_t$ is a \emph{log-concave} distribution, and such
%% distributions admit polynomial time samplers. We use Projected
%% Langevin Monte Carlo for two reasons: first, it has already been
%% analyzed by Bubeck, Eldan and Lehec~\cite{bubeck2015sampling}, and
%% second, its resemblance to stochastic gradient descent suggests that
%% it may yield a practical algorithm for non-convex classes like neural
%% networks. To prove that Projected LMC yields an efficient algorithm,
%% we use randomized smoothing and a coupling argument 


\paragraph{Langevin Monte Carlo.} The main computational insight is
that owing to the convexity properties of $\Theta$ and $f(\cdot)$, the
function $F_t$ is convex, so $P_t$ is \emph{log-concave}. Such
distributions admit polynomial time sampling routines, and 
we use
Projected Langevin Monte Carlo (LMC), which has been analyzed by
Bubeck, Eldan and Lehec~\cite{bubeck2015sampling}. To sample from
$P_t$, Projected LMC defines a Markov chain, with $\theta_0 = 0$, via
the update
\begin{align*}
  \theta_{k} = \Pcal_{\Theta}\left(\theta_{k-1} - \frac{\alpha}{2}\nabla F_t(\theta_{k-1}) + \sqrt{\alpha}\xi_{k-1}\right),
\end{align*}
where $\xi_1,\xi_2,\ldots,$ are a sequence of independent
$\Ncal(0,I_d)$ random vectors. Intuitively, $\theta_k$ converges
toward the minimizer of $F_t$, but the Gaussian noise term results in
a stationary distribution with significant mass near the
minimizer. Indeed, if $F_t$ is smooth (i.e. its gradient is Lipschitz
continuous), the stationary distribution of Projected LMC is exactly
$P_t$.

Unfortunately, $F_t$ is \emph{not} smooth in our case since
$\hinge(s)$ is non-differentiable at $s=-\gamma$, so previous analysis
of LMC do not apply. Nevertheless, using randomized
smoothing~\cite{duchi2012randomized}, and a coupling argument, we
prove that Algorithm~\ref{alg:lmc} runs in polynomial time and
generates a sample from a distribution that is close (in Wasserstein
distance) to $P_t$. This guarantee suffices for our regret analysis.

% Resolving this issue requires significant
% technical work: we use randomized smoothing~\cite{duchi2012randomized}
% to define a smoothed and strongly convex potential
% $\hat{F}_t(\theta) = \EE_{Z}F_t(\theta + Z) + \lambda \|\theta\|_2^2$
% where $Z$ is a suitably chosen random variable, and then further
% approximate $\hat{F}_t$ by sampling $Z$ so that we can compute
% gradients efficiently. In our proof, we use a coupling argument to
% show that running Projected-LMC on the sampled approximation closely
% tracks the iterates on $\hat{F}_t$, which itself provides a suitable
% approximation to $F_t$. All told, this yields a polynomial time
% algorithm for sampling from a distribution that is close (in
% Wasserstein distance) to $P_t$, which is sufficient for our regret
% analysis.

\paragraph{Calibration and Variance Control.} Statistically, the key
insight is that the hinge surrogate losses also naturally control the
variance term in the Hedge regret bound. To do so, we must define the
induced policy distribution $\pi_\theta: \Xcal \to \Delta(\Acal)$, via
$\pi_\theta(x,a) \propto \hinge(f(x,a;\theta))$. At iteration $t$, the
algorithm runs Projected LMC to obtain a sample $\theta_t$ and then
chooses an action by further sampling $a_t \sim \pi_{\theta_t}(x_t)$

By Lemma 1, this
definition lets us upper bound the algorithm's cost-sensitive loss by
the hinge loss, but more importantly, it controls the variance term

\paragraph{Other elements.}
\end{comment}

To summarize, \lmc\xspace is the first $\sqrt{T}$-regret algorithm for
bandit multiclass classification using the hinge loss. It also
represents a new approach to adversarial contextual bandits, again
with $\sqrt{T}$-regret against convex policy classes (with
realizability). Finally, while we lose the theoretical guarantees, the
algorithm easily extends to non-convex classes, which we expect to be
practically effective.



\subsection{Smooth-FTL}
\label{ssec:ftl}

Our second algorithm is simply Follow-The-Leader with uniform
smoothing, which we call \ftl. Here we return to the abstract setting with regression
class $\Fcal$. At each round $t$, we compute the empirical hinge-loss
minimizer
\begin{align*}
\hat{f}_t = \argmin_{f \in \Fcal}\sum_{\tau=1}^{t-1} \langle \hat{\ell}_\tau, \hinge(f(x_\tau))\rangle,
\end{align*}
and we choose $a_t$ from $p_t = (1 - K\mu)\pihinge(\hat{f}_t(x_t)) +
\mu$. This algorithm requires solving one hinge-loss minimization
problem at each round, and hence is efficient for many classes of
interest. Moreover, it enjoys the following regret guarantee.
\begin{theorem}[\ftl\xspace Regret Bound]
\label{thm:ftl}
Suppose that $\Fcal$ satisfies $\log
\Ncal_{\infty,\infty}(\epsilon,\Fcal) \leq \epsilon^{-p}$ for some $p
> 2$. Then in the stochastic setting, with $\mu = T^{\frac{-1}{p+1}}$,
\ftl\xspace enjoys the following expected regret guarantee
\begin{align*}
  \sum_{t=1}^T \EE \ell_t(a_t) \leq \inf_{f \in \Fcal} T \EE \langle \ell, \hinge(f(x))\rangle + \otil\left(K (T/\gamma)^{\frac{p}{p+1}}\right).
\end{align*}
\end{theorem}
This provides an algorithmic counterpart to
Theorem~\ref{thm:adaptive_minimax} in the $p \ge 2$ regime. Curiously,
this shows that for large nonparametric classes (with $\epsilon^{-p},
p > 2$ type metric entropy), sophisticated exploration is not
necessary \akshay{Only with a lower bound!!}. This also improves on
several results for bandit non-parametric learning that achieve
$\otil(T^{\frac{p+1}{p+2}})$ regret in the special case of Lipschitz
functions.


\section{Discussion}

